Automatizing Software Cognitive Complexity Reduction through Integer Linear Programming

Reducing the cognitive complexity of a piece of code to a given threshold is not trivial. Recently, we modeled software cognitive complexity reduction as an optimization problem and we proposed an approach to assist developers on this task. This approach enumerates sequences of code extraction refactoring operations until a stopping criterion is met. As a result, it returns the minimal sequence of code extraction refactoring operations that is able to reduce the cognitive complexity of a code to the given threshold. However, exhaustive enumeration algorithms fail to scale with the code size. The number of refactoring plans can grow exponentially with the number of lines of code. In this paper, instead of enumerating sequences of code extraction refactoring operations, we model the cognitive complexity reduction as an Integer Linear Programming problem. This opens the door to the use of efficient solvers to find optimal solutions in large programs.

==> includes/biography.tex <==
\clearpage
\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in]{images/ruben.jpg}}]{Dr. Rub\'en Saborido} is a researcher at the Networking and Emerging Optimization group at the Department of Computer Science at University of Málaga (Spain). He received his BS. degree in Computer Engineering and his MS. in Software Engineering and Artificial Intelligence from University of Malaga (Spain), where he worked for three years as a researcher assistant. In 2017, Rubén received a Ph.D. in Computer Engineering from Polytechnique Montréal (Canada) and his thesis was nominated for best thesis award. In 2018, he held a postdoctoral fellowship at Concordia University (Canada), where he worked on search-based software engineering for the Internet of Things (IoT). He was awarded in 2020 a Juan de la Cierva grant, funded by the Spanish State Research Agency, and ranked in the TOP 5 of the candidates in the Information and Communications Technologies area. Rubén's research focuses on search-based software engineering. He is also interested in the use of metaheuristics to solve multidisciplinary real-world problems of interest to our society and computer science. He has published several papers in ISI indexed journals (such as EMSE, IEEE TSE, Evolutionary Computation, and Swarm and Evolutionary Computation) and conference papers in IEEE ICPC, MCDM, IEEE SANER, and ACM ESEC/FSE. Rubén has co-organized the International Conference on Multiple Criteria Decision Making, in 2013. He is on the organizing committee of the 1st, 2nd, 3rd, and 4th International Workshop on Software Engineering Research \& Practices for the Internet of Things (SERP4IoT), co-located with ICSE 2019, ICSE 2020, and ICSE 2021, and ICSE 2022, respectively. He is also on the program committee of the Real World Applications (RWA) track of the Genetic and Evolutionary Computation Conference (GECCO), from 2016 up today. Rubén also acts as a reviewer of prestigious international journals (ISI / JCR).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{images/ferrer.jpg}}]{Dr. Javier Ferrer} obtained his PhD in Computer Engineering at the University of Málaga at the beginning of 2016, having obtained a national FPI (Training of Research Staff) fellowship. He also holds two postgraduate certificates of the same University; Master in Software Engineering and Artificial Intelligence and Pedagogical Aptitude Certificate. Previously, he studied Computer Science and Technical Computer Science. 

His research lines are mainly related to optimization techniques, particularly with the use of artificial intelligence techniques applied to the fields of Software Engineering and, recently, of Smart Cities. His research works have materialized in publications in international journals (10), book chapters (3), and international and national conference proceedings (28). Some of these works have been developed in collaboration with other research groups in countries such as Germany, Austria or Mexico. Dr. Ferrer has been member of the research team in 4 national projects, 3 regional project, 4 project funded by the University of Málaga and 10 contracts with companies and institutions for transference of knowledge (OTRI). He also acts as a reviewer of prestigious international journals (ISI / JCR). His H index is currently 12 with 503 cites to his works.
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{images/francis.jpeg}}]{Dr. Francisco Chicano} holds a PhD in Computer Science from the University of Málaga and a Degree in Physics from the National Distance Education University. Since 2008 he is with the Department of Languages and Computing Sciences of the University of Málaga. His research interests include the application of search techniques to Software Engineering problems and the use of theoretical results to efficiently solve combinatorial optimization problems. He is in the editorial board of Evolutionary Computation Journal, Engineering Applications of Artificial Intelligence, Journal of Systems and Software, ACM Transactions on Evolutionary Learning and Optimization and Mathematical Problems in Engineering. He has also been program chair and Editor-in-Chief in international events. 
\end{IEEEbiography}
